Classification with Valid and Adaptive Coverage

Conformal inference, cross-validation+, and the jackknife+ are hold-out methods that can be combined with virtually any machine learning algorithm to construct prediction sets with guaranteed marginal coverage. In this paper, we develop specialized versions of these techniques for categorical and unordered response labels that, in addition to providing marginal coverage, are also fully adaptive to complex data distributions, in the sense that they perform favorably in terms of approximate conditional coverage compared to alternative methods. The heart of our contribution is a novel conformity score, which we explicitly demonstrate to be powerful and intuitive for classification problems, but whose underlying principle is potentially far more general. Experiments on synthetic and real data demonstrate the practical value of our theoretical guarantees, as well as the statistical advantages of the proposed methods over the existing alternatives.

==> tables/summary_cifar10.tex <==

\begin{tabular}{c>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Coverage} & \multicolumn{6}{c}{Conditional coverage} & \multicolumn{6}{c}{Size | coverage} \\
\cmidrule(l{3pt}r{3pt}){2-7} \cmidrule(l{3pt}r{3pt}){8-13} \cmidrule(l{3pt}r{3pt}){14-19}
Black box & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC\\
\midrule
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{500}}\\
\hspace{1em}NNet & 0.91 (0.02) & 0.94 (0.01) & 0.92 (0.01) & 0.90 (0.02) & 0.90 (0.03) & 0.90 (0.02) & 0.88 (0.03) & \textcolor{green}{0.93 (0.02)} & \textcolor{green}{0.90 (0.02)} & \textcolor{red}{0.77 (0.06)} & \textcolor{red}{0.80 (0.06)} & \textcolor{red}{0.85 (0.04)} & 8.21 (0.37) & 8.43 (0.23) & \textcolor{blue}{7.99 (0.25)} & 9.55 (0.16) & 9.37 (0.19) & 9.05 (0.28)\\
\hspace{1em}RFC & 0.90 (0.02) & 0.96 (0.01) & 0.96 (0.01) & 0.91 (0.02) & 0.90 (0.03) & 0.90 (0.02) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.96 (0.01)} & \textcolor{green}{0.96 (0.02)} & \textcolor{red}{0.79 (0.06)} & \textcolor{red}{0.84 (0.05)} & \textcolor{green}{0.90 (0.03)} & 7.80 (0.36) & 8.23 (0.32) & 8.11 (0.34) & 9.43 (0.44) & 8.67 (0.40) & \textcolor{blue}{7.67 (0.37)}\\
\hspace{1em}SVC & 0.90 (0.02) & 0.93 (0.01) & 0.91 (0.02) & 0.90 (0.03) & 0.90 (0.02) & 0.90 (0.02) & 0.89 (0.03) & \textcolor{green}{0.92 (0.02)} & 0.89 (0.03) & \textcolor{red}{0.80 (0.06)} & \textcolor{red}{0.82 (0.05)} & \textcolor{red}{0.87 (0.03)} & 7.92 (0.37) & 7.88 (0.32) & \textcolor{blue}{7.41 (0.38)} & 9.39 (0.47) & 8.75 (0.41) & 7.83 (0.33)\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{1000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.96 (0.01) & 0.93 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & 0.88 (0.03) & \textcolor{green}{0.95 (0.01)} & \textcolor{green}{0.92 (0.02)} & \textcolor{red}{0.77 (0.04)} & \textcolor{red}{0.82 (0.04)} & \textcolor{red}{0.86 (0.03)} & \textcolor{blue}{7.78 (0.25)} & 8.08 (0.18) & 7.82 (0.17) & 9.47 (0.16) & 9.19 (0.15) & 8.80 (0.23)\\
\hspace{1em}RFC & 0.90 (0.01) & 0.96 (0.01) & 0.96 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.96 (0.01)} & \textcolor{green}{0.96 (0.01)} & \textcolor{red}{0.80 (0.06)} & \textcolor{red}{0.84 (0.04)} & \textcolor{green}{0.90 (0.02)} & 7.11 (0.31) & 7.55 (0.24) & 7.47 (0.24) & 9.43 (0.45) & 8.16 (0.42) & \textcolor{blue}{6.90 (0.30)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.92 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & 0.88 (0.02) & \textcolor{green}{0.92 (0.02)} & 0.89 (0.02) & \textcolor{red}{0.80 (0.05)} & \textcolor{red}{0.82 (0.04)} & 0.88 (0.03) & 7.35 (0.27) & 7.18 (0.23) & \textcolor{blue}{6.75 (0.24)} & 9.40 (0.42) & 8.58 (0.43) & 7.22 (0.31)\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{5000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.96 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.96 (0.01)} & NA & \textcolor{red}{0.79 (0.05)} & \textcolor{red}{0.84 (0.03)} & \textcolor{red}{0.86 (0.02)} & \textcolor{blue}{7.09 (0.14)} & 7.25 (0.12) & NA & 9.16 (0.20) & 8.40 (0.14) & 7.86 (0.19)\\
\hspace{1em}RFC & 0.90 (0.01) & 0.95 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.94 (0.01)} & NA & \textcolor{red}{0.82 (0.04)} & \textcolor{red}{0.86 (0.03)} & \textcolor{green}{0.90 (0.02)} & 6.03 (0.15) & 6.36 (0.11) & NA & 8.81 (0.51) & 7.33 (0.29) & \textcolor{blue}{5.81 (0.15)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.90 (0.02)} & NA & \textcolor{red}{0.81 (0.04)} & \textcolor{red}{0.84 (0.03)} & 0.89 (0.02) & 6.09 (0.12) & 5.99 (0.10) & NA & 8.84 (0.41) & 7.75 (0.29) & \textcolor{blue}{5.96 (0.12)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{10000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.96 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.95 (0.01)} & NA & \textcolor{red}{0.81 (0.05)} & \textcolor{red}{0.85 (0.03)} & \textcolor{red}{0.87 (0.02)} & 5.99 (0.16) & \textcolor{blue}{5.89 (0.09)} & NA & 8.89 (0.26) & 7.92 (0.12) & 5.93 (0.24)\\
\hspace{1em}RFC & 0.90 (0.01) & 0.94 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.94 (0.01)} & NA & \textcolor{red}{0.83 (0.04)} & \textcolor{red}{0.86 (0.03)} & 0.89 (0.02) & 5.69 (0.09) & 5.99 (0.05) & NA & 8.18 (0.63) & 7.13 (0.22) & \textcolor{blue}{5.44 (0.09)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.91 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & 0.89 (0.02) & NA & \textcolor{red}{0.82 (0.03)} & \textcolor{red}{0.84 (0.03)} & 0.89 (0.02) & 5.87 (0.08) & 5.83 (0.06) & NA & 8.37 (0.48) & 7.66 (0.18) & \textcolor{blue}{5.74 (0.08)}\\
\bottomrule
\end{tabular}

==> tables/summary_fashion.tex <==

\begin{tabular}{c>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Coverage} & \multicolumn{6}{c}{Conditional coverage} & \multicolumn{6}{c}{Size | coverage} \\
\cmidrule(l{3pt}r{3pt}){2-7} \cmidrule(l{3pt}r{3pt}){8-13} \cmidrule(l{3pt}r{3pt}){14-19}
Black box & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC\\
\midrule
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{500}}\\
\hspace{1em}NNet & 0.90 (0.02) & 0.92 (0.01) & 0.90 (0.01) & 0.91 (0.03) & 0.91 (0.02) & 0.90 (0.02) & \textcolor{red}{0.86 (0.04)} & 0.88 (0.03) & \textcolor{red}{0.86 (0.03)} & \textcolor{red}{0.79 (0.06)} & \textcolor{red}{0.85 (0.04)} & \textcolor{red}{0.85 (0.04)} & 2.97 (0.78) & 1.96 (0.22) & \textcolor{blue}{1.82 (0.17)} & 6.59 (1.24) & 3.59 (0.69) & 2.60 (0.55)\\
\hspace{1em}RFC & 0.90 (0.02) & 0.92 (0.01) & 0.92 (0.01) & 0.90 (0.03) & 0.90 (0.02) & 0.91 (0.02) & 0.88 (0.03) & \textcolor{green}{0.91 (0.02)} & \textcolor{green}{0.90 (0.02)} & \textcolor{red}{0.76 (0.07)} & \textcolor{red}{0.82 (0.06)} & \textcolor{red}{0.86 (0.05)} & 2.47 (0.24) & 2.28 (0.11) & 2.23 (0.10) & 6.68 (1.77) & 3.95 (0.83) & \textcolor{blue}{1.98 (0.22)}\\
\hspace{1em}SVC & 0.90 (0.02) & 0.93 (0.01) & 0.90 (0.02) & 0.90 (0.03) & 0.90 (0.02) & 0.90 (0.02) & \textcolor{red}{0.86 (0.03)} & \textcolor{green}{0.91 (0.02)} & 0.88 (0.03) & \textcolor{red}{0.76 (0.06)} & \textcolor{red}{0.80 (0.05)} & \textcolor{red}{0.84 (0.05)} & 2.74 (0.29) & 2.43 (0.13) & 2.30 (0.14) & 6.61 (1.41) & 4.87 (0.80) & \textcolor{blue}{2.15 (0.29)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{1000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.93 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & \textcolor{red}{0.85 (0.04)} & \textcolor{green}{0.91 (0.02)} & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.81 (0.06)} & \textcolor{red}{0.85 (0.04)} & \textcolor{red}{0.85 (0.04)} & 1.82 (0.21) & 1.71 (0.06) & \textcolor{blue}{1.53 (0.05)} & 5.73 (1.57) & 2.13 (0.31) & 1.72 (0.15)\\
\hspace{1em}RFC & 0.90 (0.01) & 0.92 (0.01) & 0.91 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.01) & 0.89 (0.03) & \textcolor{green}{0.91 (0.02)} & \textcolor{green}{0.90 (0.02)} & \textcolor{red}{0.77 (0.06)} & \textcolor{red}{0.84 (0.04)} & \textcolor{red}{0.85 (0.04)} & 2.20 (0.13) & 2.11 (0.07) & 2.09 (0.07) & 5.88 (1.73) & 2.70 (0.55) & \textcolor{blue}{1.64 (0.10)}\\
\hspace{1em}SVC & 0.90 (0.02) & 0.92 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & 0.88 (0.02) & \textcolor{green}{0.91 (0.02)} & 0.88 (0.02) & \textcolor{red}{0.78 (0.05)} & \textcolor{red}{0.83 (0.04)} & \textcolor{red}{0.85 (0.04)} & 2.30 (0.13) & 2.11 (0.07) & 2.01 (0.08) & 5.89 (1.60) & 3.26 (0.54) & \textcolor{blue}{1.71 (0.12)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{5000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.94 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{red}{0.86 (0.03)} & \textcolor{green}{0.93 (0.02)} & NA & \textcolor{red}{0.84 (0.04)} & \textcolor{red}{0.86 (0.03)} & \textcolor{red}{0.86 (0.03)} & 1.35 (0.02) & 1.45 (0.02) & NA & 3.29 (1.40) & 1.36 (0.05) & \textcolor{blue}{1.29 (0.04)}\\
\hspace{1em}RFC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.91 (0.02)} & NA & \textcolor{red}{0.81 (0.06)} & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.86 (0.03)} & 1.92 (0.04) & 1.87 (0.02) & NA & 3.91 (1.50) & 1.65 (0.10) & \textcolor{blue}{1.32 (0.03)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.91 (0.02)} & NA & \textcolor{red}{0.82 (0.04)} & \textcolor{red}{0.85 (0.03)} & \textcolor{red}{0.85 (0.03)} & 1.76 (0.04) & 1.67 (0.03) & NA & 3.49 (1.23) & 1.74 (0.16) & \textcolor{blue}{1.29 (0.03)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{10000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.94 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.88 (0.03) & \textcolor{green}{0.94 (0.02)} & NA & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.86 (0.03)} & \textcolor{red}{0.86 (0.03)} & 1.31 (0.02) & 1.43 (0.02) & NA & 1.47 (0.38) & 1.26 (0.03) & \textcolor{blue}{1.22 (0.02)}\\
\hspace{1em}RFC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.91 (0.02)} & NA & \textcolor{red}{0.86 (0.04)} & 0.88 (0.03) & \textcolor{red}{0.87 (0.03)} & 1.83 (0.03) & 1.79 (0.02) & NA & 2.20 (0.90) & 1.49 (0.06) & \textcolor{blue}{1.25 (0.02)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.89 (0.02) & \textcolor{green}{0.90 (0.02)} & NA & \textcolor{red}{0.85 (0.03)} & \textcolor{red}{0.86 (0.03)} & \textcolor{red}{0.86 (0.03)} & 1.63 (0.03) & 1.57 (0.02) & NA & 1.85 (0.72) & 1.40 (0.06) & \textcolor{blue}{1.21 (0.02)}\\
\bottomrule
\end{tabular}

==> tables/summary_mice.tex <==

\begin{tabular}{c>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Coverage} & \multicolumn{6}{c}{Conditional coverage} & \multicolumn{6}{c}{Size | coverage} \\
\cmidrule(l{3pt}r{3pt}){2-7} \cmidrule(l{3pt}r{3pt}){8-13} \cmidrule(l{3pt}r{3pt}){14-19}
Black box & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC\\
\midrule
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{500}}\\
\hspace{1em}NNet & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.02) & 0.91 (0.03) & 0.91 (0.02) & 0.89 (0.06) & \textcolor{green}{0.91 (0.05)} & \textcolor{green}{0.91 (0.06)} & \textcolor{red}{0.79 (0.11)} & \textcolor{red}{0.81 (0.10)} & \textcolor{red}{0.83 (0.09)} & 1.11 (0.03) & 1.04 (0.01) & 1.03 (0.01) & 1.96 (1.23) & 1.08 (0.10) & \textcolor{blue}{1.00 (0.00)}\\
\hspace{1em}RFC & 0.90 (0.02) & 0.92 (0.02) & 0.91 (0.02) & 0.90 (0.02) & 0.91 (0.02) & 0.90 (0.02) & \textcolor{red}{0.86 (0.07)} & \textcolor{green}{0.91 (0.05)} & 0.89 (0.06) & \textcolor{red}{0.78 (0.12)} & \textcolor{red}{0.83 (0.09)} & \textcolor{red}{0.80 (0.10)} & 1.54 (0.12) & 1.36 (0.05) & 1.30 (0.05) & 3.43 (1.33) & 1.95 (0.33) & \textcolor{blue}{1.22 (0.09)}\\
\hspace{1em}SVC & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.03) & 0.90 (0.03) & 0.90 (0.02) & 0.89 (0.06) & \textcolor{green}{0.90 (0.06)} & \textcolor{green}{0.90 (0.05)} & \textcolor{red}{0.78 (0.12)} & \textcolor{red}{0.80 (0.11)} & \textcolor{red}{0.80 (0.10)} & 1.22 (0.06) & 1.08 (0.02) & 1.07 (0.02) & 1.93 (1.24) & 1.05 (0.07) & \textcolor{blue}{1.00 (0.00)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{1000}}\\
\hspace{1em}NNet & 0.89 (0.02) & 0.91 (0.02) & 0.91 (0.04) & 0.90 (0.04) & 0.90 (0.03) & 0.90 (0.02) & NA (NA) & \textcolor{green}{0.91 (0.13)} & NA (NA) & \textcolor{green}{0.91 (0.11)} & NA (NA) & NA (NA) & 1.03 (0.02) & 1.01 (0.01) & 1.01 (0.01) & \textcolor{blue}{1.00 (0.00)} & 1.00 (0.00) & 1.00 (0.00)\\
\hspace{1em}RFC & 0.90 (0.03) & 0.90 (0.03) & 0.89 (0.03) & 0.89 (0.04) & 0.89 (0.04) & 0.90 (0.03) & NA (NA) & NA (NA) & NA (NA) & \textcolor{green}{0.92 (0.13)} & NA (NA) & NA (NA) & 1.31 (0.06) & 1.19 (0.04) & 1.17 (0.06) & 1.92 (0.79) & 1.19 (0.10) & \textcolor{blue}{1.01 (0.01)}\\
\hspace{1em}SVC & 0.89 (0.04) & 0.90 (0.03) & 0.90 (0.03) & 0.90 (0.03) & 0.91 (0.04) & 0.90 (0.03) & NA (NA) & NA (NA) & NA (NA) & NA (NA) & NA (NA) & NA (NA) & 1.06 (0.04) & 1.02 (0.02) & 1.02 (0.02) & 1.10 (0.65) & \textcolor{blue}{1.00 (0.00)} & 1.00 (0.00)\\
\bottomrule
\end{tabular}

==> tables/summary_mnist.tex <==

\begin{tabular}{c>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Coverage} & \multicolumn{6}{c}{Conditional coverage} & \multicolumn{6}{c}{Size | coverage} \\
\cmidrule(l{3pt}r{3pt}){2-7} \cmidrule(l{3pt}r{3pt}){8-13} \cmidrule(l{3pt}r{3pt}){14-19}
Black box & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC & SC & CV+ & JK+ & CQC & CQC-RF & HCC\\
\midrule
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{500}}\\
\hspace{1em}NNet & 0.90 (0.02) & 0.92 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.02) & \textcolor{red}{0.85 (0.04)} & \textcolor{green}{0.90 (0.03)} & 0.88 (0.03) & \textcolor{red}{0.81 (0.05)} & \textcolor{red}{0.86 (0.04)} & \textcolor{red}{0.86 (0.04)} & 2.51 (0.68) & 1.67 (0.08) & \textcolor{blue}{1.54 (0.07)} & 6.63 (1.29) & 3.17 (0.61) & 2.25 (0.39)\\
\hspace{1em}RFC & 0.91 (0.02) & 0.93 (0.01) & 0.92 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.02) & 0.88 (0.03) & 0.88 (0.03) & 0.88 (0.03) & \textcolor{red}{0.80 (0.07)} & \textcolor{red}{0.85 (0.04)} & \textcolor{red}{0.86 (0.03)} & 2.55 (0.33) & 2.21 (0.13) & 2.15 (0.13) & 7.14 (1.77) & 4.02 (0.89) & \textcolor{blue}{2.06 (0.31)}\\
\hspace{1em}SVC & 0.90 (0.02) & 0.92 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.02) & \textcolor{red}{0.87 (0.04)} & \textcolor{green}{0.91 (0.02)} & 0.89 (0.02) & \textcolor{red}{0.79 (0.05)} & \textcolor{red}{0.83 (0.05)} & \textcolor{red}{0.85 (0.04)} & 2.51 (0.29) & 2.19 (0.12) & 2.06 (0.13) & 6.68 (1.52) & 3.97 (0.89) & \textcolor{blue}{1.91 (0.31)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{1000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.93 (0.01) & 0.91 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & 0.88 (0.03) & \textcolor{green}{0.92 (0.02)} & \textcolor{green}{0.90 (0.02)} & \textcolor{red}{0.83 (0.05)} & \textcolor{red}{0.86 (0.04)} & \textcolor{red}{0.86 (0.03)} & 1.53 (0.09) & 1.43 (0.04) & \textcolor{blue}{1.29 (0.03)} & 5.37 (1.47) & 1.74 (0.24) & 1.36 (0.11)\\
\hspace{1em}RFC & 0.90 (0.01) & 0.92 (0.01) & 0.92 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & \textcolor{red}{0.87 (0.03)} & 0.88 (0.03) & 0.88 (0.03) & \textcolor{red}{0.81 (0.05)} & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.86 (0.04)} & 2.07 (0.13) & 1.99 (0.08) & 1.96 (0.08) & 6.17 (1.59) & 2.47 (0.44) & \textcolor{blue}{1.53 (0.13)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.92 (0.01) & 0.90 (0.01) & 0.90 (0.02) & 0.90 (0.02) & 0.90 (0.01) & 0.89 (0.03) & \textcolor{green}{0.92 (0.02)} & \textcolor{green}{0.90 (0.02)} & \textcolor{red}{0.81 (0.04)} & \textcolor{red}{0.86 (0.04)} & \textcolor{red}{0.86 (0.03)} & 2.07 (0.11) & 1.91 (0.08) & 1.82 (0.08) & 5.63 (1.58) & 1.89 (0.36) & \textcolor{blue}{1.37 (0.11)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{5000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.92 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.92 (0.01)} & NA & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.87 (0.03)} & 0.88 (0.03) & 1.13 (0.01) & 1.14 (0.01) & NA & 1.14 (0.46) & 1.02 (0.02) & \textcolor{blue}{1.00 (0.00)}\\
\hspace{1em}RFC & 0.90 (0.01) & 0.91 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{red}{0.87 (0.03)} & 0.89 (0.02) & NA & \textcolor{red}{0.85 (0.04)} & 0.88 (0.02) & \textcolor{red}{0.87 (0.03)} & 1.80 (0.05) & 1.76 (0.03) & NA & 3.05 (1.19) & 1.27 (0.06) & \textcolor{blue}{1.11 (0.02)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.91 (0.02)} & NA & \textcolor{red}{0.85 (0.04)} & \textcolor{red}{0.87 (0.02)} & \textcolor{red}{0.87 (0.03)} & 1.61 (0.04) & 1.50 (0.03) & NA & 1.96 (1.28) & 1.09 (0.02) & \textcolor{blue}{1.05 (0.01)}\\
\addlinespace[0.3em]
\multicolumn{19}{l}{\textbf{10000}}\\
\hspace{1em}NNet & 0.90 (0.01) & 0.92 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.92 (0.01)} & NA & \textcolor{red}{0.87 (0.02)} & \textcolor{red}{0.87 (0.02)} & \textcolor{red}{0.87 (0.02)} & 1.07 (0.01) & 1.10 (0.01) & NA & \textcolor{blue}{1.00 (0.00)} & 1.00 (0.00) & 1.00 (0.00)\\
\hspace{1em}RFC & 0.90 (0.01) & 0.91 (0.00) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & 0.88 (0.02) & 0.89 (0.02) & NA & \textcolor{red}{0.87 (0.03)} & 0.88 (0.02) & \textcolor{red}{0.87 (0.03)} & 1.74 (0.03) & 1.70 (0.02) & NA & 1.59 (0.60) & 1.13 (0.02) & \textcolor{blue}{1.05 (0.01)}\\
\hspace{1em}SVC & 0.90 (0.01) & 0.91 (0.01) & NA & 0.90 (0.01) & 0.90 (0.01) & 0.90 (0.01) & \textcolor{green}{0.90 (0.02)} & \textcolor{green}{0.91 (0.02)} & NA & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.87 (0.03)} & \textcolor{red}{0.87 (0.03)} & 1.46 (0.02) & 1.38 (0.02) & NA & 1.07 (0.07) & 1.04 (0.01) & \textcolor{blue}{1.02 (0.00)}\\
\bottomrule
\end{tabular}
